Kac-Moody algebraic structures in supergravity theories

A lot of developments made during the last years show that Kac-Moody algebras play an important role in the algebraic structure of some supergravity theories. These algebras would generate infinite-dimensional symmetry groups. The possible existence of such symmetries have motivated the reformulation of these theories as non-linear sigma-models based on the Kac-Moody symmetry groups. Such models are constructed in terms of an infinite number of fields parametrizing the generators of the corresponding algebra. If these conjectured symmetries are indeed actual symmetries of certain supergravity theories, a meaningful question to elucidate will be the interpretation of this infinite tower of fields. Another substantial problem is to find the correspondence between the sigma-models, which are explicitly invariant under the conjectured symmetries, and these corresponding space-time theories. The subject of this thesis is to address these questions in certain cases.

==> actionsu21.tex <==
\chapter{Action of $\su$ on BPS solutions } 

